Transition Systems from Causal Reversible Bundle Event Structures

Reversible computing is a novel paradigm that has recently emerged and extends traditional forwards-only computation with the capability to execute in the reverse direction, making it possible for computation to run backwards as well as forwards. Event structures are a foundational model in concurrency theory, providing a way to understand computational processes by describing the events that occur and the relationships between them. In the literature, two structurally different approaches to associating transition system semantics with event structure models have been distinguished. One approach is based on configurations, which are sets of already executed events. The other approach is based on model residuals, which are not yet executed fragments of the model. Configuration-based transition systems appear to be primarily used for semantic representations. Residual-based transition systems are actively applied to demonstrate the consistency between operational and denotational semantics of concurrent process calculi, as well as to visualize the dynamics of models. The present paper focuses on bundle event structures with causal reversibility, which are used in the study of reversible extensions of CCS- and Ï€-like systems. Mappings from the reversible event structure model to the two transition system semantics are developed, which made it possible to prove the isomorphism of the semantics. A category-theoretic characterization of the mappings is provided.

==> eptcsdata.tex <==
\providecommand{\firstpage}{171}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.12}{10.4204/EPTCS.451.12}}
\pdfoutput=1

